Neural Rays for Occlusion-aware Image-based Rendering

We present a new neural representation, called Neural Ray (NeuRay), for the novel view synthesis task. Recent works construct radiance fields from image features of input views to render novel view images, which enables the generalization to new scenes. However, due to occlusions, a 3D point may be invisible to some input views. On such a 3D point, these generalization methods will include inconsistent image features from invisible views, which interfere with the radiance field construction. To solve this problem, we predict the visibility of 3D points to input views within our NeuRay representation. This visibility enables the radiance field construction to focus on visible image features, which significantly improves its rendering quality. Meanwhile, a novel consistency loss is proposed to refine the visibility in NeuRay when finetuning on a specific scene. Experiments demonstrate that our approach achieves state-of-the-art performance on the novel view synthesis task when generalizing to unseen scenes and outperforms per-scene optimization methods after finetuning.

==> 00_introduction_bak.tex <==
\section{Introduction}

Novel View Synthesis (NVS) is an important problem in computer graphics and computer vision. Given a set of input images with known camera poses, the goal of NVS is to synthesize images of the scene from arbitrary virtual camera poses. Recently, neural rendering methods have achieved impressive improvements on the NVS problem compared to earlier image-based rendering methods~\cite{kalantari2016learning, hedman2018deep, mildenhall2019local}. Neural Radiance Field (NeRF)~\cite{mildenhall2020nerf} shows that photo-realistic images of unseen views can be synthesized from a 5D radiance field encoded in a neural network. This neural network learns a radiance field $(\sigma,\bm{c})=f(\bm{p},\bm{r})$ which maps a position $\bm{p}$ and a direction $\bm{r}$ to a density $\sigma$ and a color $\bm{c}$. Novel views can be synthesized with a volume renderer. However, these methods cannot generalize to unseen scenes as they learn scene-specific networks, which usually take hours or days for a single scene.

Recent works like GRF~\cite{Trevithick20arxiv_GRF}, IBRNet~\cite{wang2021ibrnet}, SRF~\cite{chibane2021stereo} and PixelNeRF~\cite{Yu20arxiv_pixelNeRF} aim to design NeRF-like neural rendering frameworks that can generalize to unseen scenes. These works are motivated by traditional stereo matching methods which extract local image features on the input views and match these features to determine 3D surfaces, i.e., the density $\sigma$, on a specific 3D point, as shown in Fig.~\ref{fig:occ} (a). Then, the color $\bm{c}$ of this point is computed from features or blending colors of input views. This scheme enables these methods to generalize to unseen scenes. However, when features are inconsistent on a point, it is hard for these methods to determine whether such inconsistency is caused by occlusions as shown in Fig.~\ref{fig:occ} (b) or this point is a non-surface point as shown in Fig.~\ref{fig:occ} (c).
% Sida: 点到为止，说太多怕被相关论文的作者反对
% Especially, on datasets with fewer input views, more complex shapes and notable self-occlusions (e.g. the NeRF Synthetic dataset~\cite{mildenhall2020nerf}), these methods struggle to correctly render the novel view image even after being finetuned on the scene.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image_new/inconsistency.pdf}
    \caption{(a) Without occlusions, local image features are consistent on the surface point. (b) Local image features are inconsistent on a surface point due to occlusions. (c) Local image features are inconsistent on a non-surface point. 
    Stereo matching based rendering methods (e.g. GRF, PixelNeRF, IBRNet, and SRF) will correctly assign a large density to the surface point in (a) due to the feature consistency. However, they are unable to distinguish two feature inconsistency in (b) and (c) thus struggle to render a correct color in the cases.}
    \label{fig:occ}
\end{figure}

To overcome this limitation, we propose a new 3D representation, called {\em Neural Ray} (NeuRay), as a backend representation of the stereo matching based rendering methods. 
NeuRay depicts the scene geometry by so-called {\em reference rays}, which are camera rays emitted from the input views to the 3D space.
For each reference ray, NeuRay predicts a visibility to determine whether a 3D point at a specific depth on the ray is visible or not.
With such visibility, we can easily distinguish the feature inconsistency caused by occlusions from that caused by non-existence of surface, thus leading to more accurate description of scene geometry and much better rendering quality on difficult scenes with severe self-occlusions.


To efficiently compute the visibility of a camera ray to any 3D point, NeuRay parameterizes the visibility with a probability distribution that indicates how far this camera ray can reach before hitting a surface.
By directly predicting the distribution parameters, estimating the visibility only requires one forward pass of the network.
This is much faster than NeRF \cite{mildenhall2020nerf} in which the computation of the visibility requires accumulating densities of multiple points along the camera ray.
Meanwhile, to enable NeuRay to generalize to unseen scenes, these probability distribution parameters can be instantly inferred from a cost volume construction from multi-view stereo~\cite{yao2018mvsnet}. 
Thus, rendering with NeuRay in an unseen scene can be seen as a two-stage framework. In the first stage, we predict the surfaces based on the cost volume construction. Then, the estimated surfaces enable the occlusion-aware prediction of density and colors to render novel view images. 
Moreover, when finetuning NeuRay in each scene, the probability distributions allow to memorize and refine the scene geometry to improve the occlusion inference. In contrast, stereo matching based rendering methods~\cite{Trevithick20arxiv_GRF,wang2021ibrnet,chibane2021stereo,Yu20arxiv_pixelNeRF} are still oblivious to the scene geometry in finetuning so that they still suffer from feature inconsistency caused by occlusions.

Another advantage of NeuRay is that the estimated visibility can be used to speed up the rendering process.
By a simple and efficient combination of visibility, we can compute the surface existence probability on any 3D point. This allows to quickly filter out most non-surface points and only apply networks on remaining points for rendering, which greatly speeds up the rendering in test time.

We conducted extensive experiments on three datasets, the NeRF synthetic dataset~\cite{mildenhall2020nerf}, the DTU dataset~\cite{jensen2014large} and the forward-facing LLFF dataset~\cite{mildenhall2019local}, to demonstrate the effectiveness of NeuRay. The results show that (1) without scene-specific optimization, NeuRay already produces satisfactory renderings that outperforms other generalization methods by a large margin; (2) finetuning NeuRay can produce much superior results than finetuning other generalization models and achieve even better rendering quality than NeRF~\cite{mildenhall2020nerf}.
Moreover, we also show that rendering a novel view of 800$\times$600 resolution with NeuRay costs $\sim$3 second, which is 10 times faster than other stereo matching based rendering methods. 



==> 00_introduction_bak2.tex <==
\section{Introduction}

Novel View Synthesis (NVS) is an important problem in computer graphics and computer vision. Given a set of input images with known camera poses, the goal of NVS is to synthesize images of the scene from arbitrary virtual camera poses. Recently, neural rendering methods have achieved impressive improvements on the NVS problem compared to earlier image-based rendering methods~\cite{kalantari2016learning, hedman2018deep, mildenhall2019local}. Neural Radiance Field (NeRF)~\cite{mildenhall2020nerf} shows that photo-realistic images of unseen views can be synthesized from a 5D radiance field encoded in a neural network. This neural network learns a radiance field which maps a position and a direction to a density and a color. Novel views can be synthesized with a volume renderer. However, these methods cannot generalize to unseen scenes as they learn scene-specific networks, which usually take hours or days for a single scene.

Recent works like GRF~\cite{Trevithick20arxiv_GRF}, IBRNet~\cite{wang2021ibrnet}, SRF~\cite{chibane2021stereo} and PixelNeRF~\cite{Yu20arxiv_pixelNeRF} aim to design NeRF-like neural rendering frameworks that can generalize to unseen scenes. These works are motivated by traditional stereo matching methods which extract local image features on the input views and match these features to determine 3D surfaces, i.e., the density $\sigma$, on a specific 3D point, as shown in Fig.~\ref{fig:occ} (a). Then, the color $\bm{c}$ of this point is computed from features or blending colors of input views. This scheme enables these methods to generalize to unseen scenes. However, when features are inconsistent on a point, it is hard for these methods to determine whether such inconsistency is caused by occlusions as shown in Fig.~\ref{fig:occ} (b) or this point is a non-surface point as shown in Fig.~\ref{fig:occ} (c).

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image_new/inconsistency.pdf}
    \caption{(a) Without occlusions, local image features are consistent on the surface point. (b) Local image features are inconsistent on a surface point due to occlusions. (c) Local image features are inconsistent on a non-surface point. 
    Stereo matching based rendering methods (e.g. GRF, PixelNeRF, IBRNet, and SRF) will correctly assign a large density to the surface point in (a) due to the feature consistency. However, they are unable to distinguish two feature inconsistency in (b) and (c) thus struggle to render a correct color in the cases.}
    \vspace{-10pt}
    \label{fig:occ}
\end{figure}


% characteristics of NeuRay representation / what is NeuRay
% 1) visibility can help occlusion inference
% 2) visibility can be efficiently computed
To overcome this limitation, we propose a new 3D representation, called {\em Neural Ray} (NeuRay), as a backend representation of the stereo matching based rendering methods. 
NeuRay depicts the scene geometry by so-called {\em reference rays}, which are camera rays emitted from the input views to the 3D space. On every reference ray, NeuRay associates a probability distribution encoded by learnable neural networks to indicate how far this ray can reach before hitting a surface. This probability distribution allows us to predict a visibility to determine whether a 3D point at a specific depth on this ray is visible or not. With such visibility, we can easily distinguish the feature inconsistency caused by occlusions from that caused by non-existence of surface, thus leading to more accurate description of scene geometry and much better rendering quality on difficult scenes with severe self-occlusions. Meanwhile, by directly encoding the distribution parameters with neural networks, estimating the visibility only requires one forward pass of the networks. This is much faster than NeRF \cite{mildenhall2020nerf} in which the computation of the visibility requires accumulating densities of dense sample points along the camera ray.

% NeuRay advantage in three aspects: 
% generalization/finetuning/speeding up
NeuRay improves the novel view synthesis in three aspects.
1) In generalization to unseen scenes, the probability distribution parameters in NeuRay can be instantly inferred from a cost volume construction from multi-view stereo~\cite{yao2018mvsnet}. 
Thus, rendering with NeuRay in an unseen scene can be seen as a two-stage framework. 
In the first stage, we predict the surfaces based on the cost volume construction. Then, the estimated surfaces enable the occlusion-aware prediction of density and colors to render novel view images. 
2) When finetuning NeuRay on a specific scene, we propose a novel consistency loss to refine the NeuRay representation by memorizing the predicted scene geometry. At the same time, the refined NeuRay representation will improve the accuracy of scene geometry prediction reversely by better occlusion inference. Thus, the NeuRay refinement and geometry prediction help each other, which leads to accurate depiction of the scene.
% In contrast, stereo matching based rendering methods~\cite{Trevithick20arxiv_GRF,wang2021ibrnet,chibane2021stereo,Yu20arxiv_pixelNeRF} are still oblivious to the scene geometry in finetuning so that they still suffer from feature inconsistency caused by occlusions.
3) The rendering process can be sped up by NeuRay.
By an efficient combination of probabilities in NeuRay, we can compute a surface existence probability on any 3D point, which allows to quickly filter out non-surface points and only apply networks on few remaining points for fast rendering.

We conducted extensive experiments on three datasets, the NeRF synthetic dataset~\cite{mildenhall2020nerf}, the DTU dataset~\cite{jensen2014large} and the forward-facing LLFF dataset~\cite{mildenhall2019local}, to demonstrate the effectiveness of NeuRay. The results show that 1) without scene-specific optimization, NeuRay already produces satisfactory renderings that outperforms other generalization methods by a large margin; 2) finetuning NeuRay can produce much superior results than finetuning other generalization models and achieve even better rendering quality than NeRF~\cite{mildenhall2020nerf}.
Moreover, we also show that rendering a novel view of 800$\times$600 resolution with NeuRay costs $\sim$3 second, which is 10 times faster than baseline stereo matching based rendering methods. 



==> 00_introduction_bak3.tex <==
\section{Introduction}

Novel View Synthesis (NVS) is an important problem in computer graphics and computer vision. Given a set of input images with known camera poses, the goal of NVS is to synthesize images of the scene from arbitrary virtual camera poses. Recently, neural rendering methods have achieved impressive improvements on the NVS problem compared to earlier image-based rendering methods~\cite{kalantari2016learning, hedman2018deep, mildenhall2019local}. Neural Radiance Field (NeRF)~\cite{mildenhall2020nerf} shows that photo-realistic images of novel views can be synthesized by volume rendering on a 5D \textit{radiance field} encoded in a neural network which maps a position and a direction to a density and a color. However, these methods cannot generalize to unseen scenes as they learn scene-specific networks, which usually take hours or days for a single scene.

Recent works \cite{Trevithick20arxiv_GRF, wang2021ibrnet, chibane2021stereo, Yu20arxiv_pixelNeRF} propose NeRF-like neural rendering frameworks that can generalize to unseen scenes. Given a set of input views, they construct a radiance field on-the-fly by extracting local image features on these views and matching multi-view features to predict colors and density on 3D points. This is similar to stereo matching methods \cite{schoenberger2016mvs, yao2018mvsnet} that check the multi-view feature consistency to find a surface point, as shown in Fig.~\ref{fig:occ} (a). However, when features are inconsistent on a point, it is hard for these methods to determine whether such inconsistency is caused by occlusions as shown in Fig.~\ref{fig:occ} (b) or this point is a non-surface point as shown in Fig.~\ref{fig:occ} (c).

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image_new/inconsistency.pdf}
    \caption{(a) Without occlusions, local image features are consistent on the surface point. (b) Local image features are inconsistent on a surface point due to occlusions. (c) Local image features are inconsistent on a non-surface point. 
    Stereo matching based rendering methods (e.g. GRF, PixelNeRF, IBRNet, and SRF) will correctly assign a large density to the surface point in (a) due to the feature consistency. However, they are unable to distinguish two feature inconsistency in (b) and (c) thus struggle to render a correct color in the cases.}
    \vspace{-10pt}
    \label{fig:occ}
\end{figure}

An intuitive solution to this problem is to consider the visibility of input views when checking the multi-view feature consistency. To obtain the visibility of a 3D point to a particular view, a naive way is to predict the densities along the camera ray from the view to the 3D point and then accumulate these densities to compute the transmittance as the visibility. However, computing visibility with this strategy is computationally impractical because it greatly increases the required number of network forward passes to compute densities along the camera ray.

In this paper, we propose a novel 3D representation, called Neural Ray (NeuRay), which enables efficient visibility computation in constructing radiance fields. For each camera ray of input views, NeuRay directly represents its visibility to any 3D point on this ray by a probability distribution. In contrast to the above density-based strategy, NeuRay only requires one network forward pass to compute the distribution parameters of visibility, which allows an occlusion-aware radiance field construction from multi-view features.
% allowing us to efficiently consider the visibilities of input features when predicting the colors and densities for 3D points.
Meanwhile, on an unseen scene, these distribution parameters can be effectively and instantly inferred by applying a multi-view stereo algorithm, which thus enables NeuRay generalize to new scenes.

% There are two additional advantages of NeuRay for novel view synthesis. 
Based on the probability distribution defined on the camera ray, NeuRay is able to estimate the surface location on the ray.
Meanwhile, the constructed radiance field is also able to compute surface locations on camera rays.
% Meanwhile, constructing radiance fields also depicts the scene geometry by predicting surface locations. 
Thus, in the scene-specific optimization of NeuRay, we propose a novel consistency loss to enforce the consistency between the surface locations from the NeuRay representation and those from the constructed radiance field. This loss enables the NeuRay representation to refine itself by memorizing the scene geometry predicted by the radiance field. At the same time, the memorized scene geometry in NeuRay will in turn improves the radiance field construction by providing better occlusion inference.
Another advantage is that estimating surface locations by NeuRay is efficient and can be used in speeding up the rendering process. Using the estimated surface locations, we are able to quickly filter out non-surface points  and only apply multi-view feature matching on few remaining points for fast rendering.
% First, we prove that the probability distribution in NeuRay can be used to derive the transmittance along the camera ray. The transmittance can also be obtained by accumulating the predicted densities along the ray, which establishes the relationship between the NeuRay and density field. This enables us to apply a consistency loss to the NeuRay and density field, which makes them teach the learned geometry to each other and leads to improvements on the performance of novel view synthesis. Second, NeuRay can be used to improve the rendering speed. For any 3D point, we are able to efficiently infer its density based on the probability distribution in NeuRay, which acts as the scene geometry to guide the point sampling in the volume rendering and allows us to only predict colors and densities for points that contain scene contents.

We conducted extensive experiments on three datasets, the NeRF synthetic dataset~\cite{mildenhall2020nerf}, the DTU dataset~\cite{jensen2014large} and the forward-facing LLFF dataset~\cite{mildenhall2019local}, to demonstrate the effectiveness of NeuRay. The results show that 1) without scene-specific optimization, NeuRay already produces satisfactory rendering results that outperforms other generalization methods by a large margin; 2) finetuning NeuRay can produce much superior results than finetuning other generalization models and achieve even better rendering quality than NeRF~\cite{mildenhall2020nerf}.
Moreover, we also show that rendering a novel view of 800$\times$600 resolution with NeuRay costs around 3 seconds, which is 10 times faster than baseline generalizable radiance field methods. 



==> 02_method_bak.tex <==
\section{Method}

Given a $N$ input views of a scene with known camera poses, called \textit{reference views}, our goal is to render images from arbitrary novel views, called \textit{query views}. Before introducing NeuRay, we first review the volume rendering and the stereo matching based rendering methods. 

\subsection{Volume rendering}
\label{sec:vr}
A ray is parameterized by $\bm{p}(z) =\bm{o}+z\bm{r}$, $z\in \mathbb{R}^{+}$, where $\bm{o}$ is the start point at the camera center, and $\bm{r}$ is the unit direction vector of the ray. Given a \textit{query ray} on a query view, we sample $K_q$ points $\{\bm{p}_i \equiv \bm{p}(z_i) |i=1,...,K_q\}$ with the increasing values $z_i$ along the ray. In the rendering process, following the ray casting approach in volume rendering, the color for the associated pixel is computed by
\begin{equation}
    \bm{c}_o=\sum_{i=1}^K \bm{c}_{i} h_{i},
    \label{eq:vr}
\end{equation}
where $\bm{c}_o\in \mathbb{R}^3$ is the output color, $\bm{c}_{i}$ the color of the sample point $\bm{p}_i$, and $h_{i}$ the hitting probability that the ray is not occluded by any depth up to the depth $z_i$ and hits a surface in the range $(z_i,z_{i+1})$. Thus, the hitting probability $h_{i}$ can be computed by
\begin{equation}
    h_{i}=\prod_{k=1}^{i-1} (1-\alpha_k)\alpha_i,
    \label{eq:prod}
\end{equation}
where $\alpha_i$ is the alpha value in the depth range $(z_i, z_{i+1})$. Obviously, the key to compute the output color is to determine the $\alpha_i$ and $\bm{c}_i$ for every sample point.

\subsection{Stereo matching based volume rendering}
\label{sec:stereo}
Unlike NeRF~\cite{mildenhall2020nerf} which maps the input coordinate $\bm{p}_i$ to $\bm{c}_i$ and $\alpha_i$ by a scene-specific neural network, stereo matching based methods~\cite{wang2021ibrnet,Yu20arxiv_pixelNeRF,chibane2021stereo,Trevithick20arxiv_GRF} compute the $\alpha_i$ and $\bm{c}_i$ by aggregating local features and colors from reference views so that they are able to generalize to unseen views. As shown in Fig.~\ref{fig:proj}, their structure can be summarized as, 
\begin{equation}
    \bm{f}_i = M (\{\bm{f}_{i,j}|j=1,...,N\}),
    \label{eq:agg}
\end{equation}
\begin{equation}
    \alpha_i = P (\bm{f}_i),
\end{equation}
\begin{equation}
    \bm{c}_i = B (\{\bm{f}_{i,j};\bm{f}_i;\bm{r}_{i,j} - \bm{r}_i;\bm{c}_{i,j}\}) ,
\end{equation}
where $\bm{f}_{i,j}$ is the local image feature of the sample point $\bm{p}_i$ projected on the $j$-th reference view, $M$ is a network which aggregates the features from different views to produce a feature $\bm{f}_i$, $P$ is another network checking the local feature consistency from $\bm{f}_i$ to produce the alpha value $\alpha_i$, $B$ is a color network which predict color $\bm{c}_i$ from the features $\bm{f}_{i,j}$, $\bm{f}_i$, the view direction difference $\bm{r}_{i,j}-\bm{r}_i$ and the color $\bm{c}_{i,j}$, where $\bm{r}_{i,j}$ is the view direction from $j$-th reference view to the point $\bm{p}_i$ and $\bm{c}_{i,j}$ is the color of this point projected on the reference view. Networks $(M,P)$ will assign a large alpha value $\alpha_i$ when local image features $\{\bm{f}_{i,j}\}$ are consistent and network $B$ will use the color $\bm{c}_{i,j}$ from views with consistent local features to produce the color $\bm{c}_i$. Though feature matching networks $(M,B,P)$ can generalize to unseen scenes, their performance degenerates severely when occlusions occur. In the following, we introduce the NeuRay representation to help the occlusion inference.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image_new/matching_rendering.pdf}
    \caption{Stereo matching based methods aggregate local features and colors of reference views to compute alpha values and colors of sample points on the query ray.}
    \label{fig:proj}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{image_new/pipeline_final.pdf}
    \caption{Pipeline of rendering with NeuRay representation.}
    \label{fig:pipeline}
\end{figure*}

\subsection{NeuRay representation}
\label{sec:neuray}
The target of NeuRay is to encode visibility. Specifically, given a point $\bm{p}_i$ and a reference view indexed by $j$, a visibility $v_{i,j}$ from this reference view to the point should be easily computed from NeuRay. Afterwards, such visibility will be used in Eq.~\ref{eq:agg} by $\bm{f}_i = M (\{(\bm{f}_{i,j};v_{i,j})\})$ to make $M$ occlusion-aware.

To achieve this, we represent the scene geometry with so-called \textit{reference rays} emitted from reference views. We associate a visibility feature vector $\bm{g}$ on every reference ray to encode a visibility function $v(z)$, which means the probability that a point at depth $z$ is visible or not for this reference ray. In this case, $v_{i,j}\equiv v_{i,j}(z_{i,j})$ where $z_{i,j}$ is the depth of the point $\bm{p}_i$ on the reference ray. Obviously, a valid visibility function $v(z)$ should be non-increasing on $z$ and $0\le v(z)\le 1$. In the following, we discuss two ways to parameterize the visibility $v(z)$ from $\bm{g}$. Then, we will illustrate how to compute $\bm{g}$ in Sec.~\ref{sec:gen} and Sec.~\ref{sec:ft}.

\textbf{Visibility from density}. Straightforwardly parameterizing visibility with a NeRF~\cite{mildenhall2020nerf}-like density is computationally intractable. In this formulation, we directly decode a density $d(z)=\phi(z;\bm{g})$ from $\bm{g}$ using a MLP $\phi$. To compute the visibility $v(z)$, we need to first sample $K_r$ depth $\{z_k\}$ with $z_k<z$, compute their densities $d(z_k)$ and the corresponding alpha values $\alpha_{k}=1-\exp(-{\rm ReLU}(d_k))$, and finally get visibility $v(z)=\prod_{k=1}^{K_r} (1-\alpha_k)$. Though the formulation is a valid visibility function, it is computationally infeasible because it requires $K_r$ times evaluation of $\phi$ to compute the visibility of a reference view to a point. 

\textbf{Visibility from occlusion probability}. Instead of using density to compute visibility, we compute the visibility from a Cumulative Density Function (CDF) $t(z)$ by $v(z)=1-t(z)$. As a CDF, $t(z)$ is non-decreasing from 0 to 1 which also forms a valid visibility function. $t(z)$ actually corresponds to a \textit{occlusion probability} that the ray is occluded before a depth $z$ and $t(z_i)-t(z_{i-1})$ is a hitting probability that the ray hits a surface in the range $(z_{i-1},z_{i})$. We parameterize $t(z)$ by a mixture of logistics distributions,
\begin{equation}
    t(z;\{\mu_i,\sigma_i,w_i\})=\sum_i^{N_{l}} w_i S((z-\mu_i)/\sigma_i),
\end{equation}
where we mix $N_{l}$ logistics distributions, $\mu_i$ is the mean of $i$-th logistics distribution, $\sigma_i$ the standard deviation, $w_i$ the mixing weight with $\sum_i w_i=1$, $S(\cdot)$ a sigmoid function. All parameters $[\mu_i,\sigma_i,w_i]$ are decoded from the visibility feature $\bm{g}$ by a MLP $\phi$. In this formulation, the visibility can be computed from a single evaluation of the network $\phi$. In general, a ray will only hit one surface so one logistics distribution will be enough. However, using a mixture of logistics distribution improves performance when the ray hits on semi-transparent surfaces or edges of surfaces. 

\subsection{Generalize with NeuRay}
\label{sec:gen}
\textbf{Pipeline}. The visibility feature $\bm{g}$ is scene-specific, but we can initialize it via a cost volume construction, which provides a coarse estimation of surface locations for the initialization of visibility in NeuRay, so that NeuRay is able to generalize to unseen scenes. 
The pipeline is shown in Fig.~\ref{fig:pipeline}. 
For every reference view with its $N_s$ neighboring reference views, we compute their feature consistency in the view frustum to construct a cost volume with size $H\times W \times D$~\cite{yao2018mvsnet}. Then, an initialization network processes the cost volume and image features to output a visibility feature map $\bm{G}'$. Such a visibility feature map is concatenated with image features and processed by another CNN, called visibility encoder, to produce a refined visibility feature map $\bm{G}\in \mathbb{R}^{H\times W\times C}$. The initialized feature vector $\bm{g}\in \mathbb{R}^C$ for a specific reference ray is computed by bilinear interpolation on the feature map $\bm{G}$, which is subsequently utilized by the decoder MLP $\phi$ to compute the visibility (Sec.~\ref{sec:neuray}). Finally, on every sample point, visibilities, colors and local features from all reference views are aggregated by feature matching networks $(M,B,P)$ to produce a alpha value and a color (Sec.~\ref{sec:stereo}), which are finally processed by the volume rendering to compute the output color (Sec.~\ref{sec:vr}). 
% Optionally, we can replace the cost volume construction with the patch match stereo~\cite{schonberger2016pixelwise} to estimate a coarse depth map and feed the estimated depth to the initialization network to initialize NeuRay. 


\textbf{Loss}. To train the generalization model, we randomly select a query view and some reference views in a training scene to render the query view with a render loss
\begin{equation}
    \ell_{render}=\sum \|\bm{c}_{o} - \bm{c}_{gt}\|^2,
\end{equation}
where $\bm{c}_{o}$ is computed by Eq.~\ref{eq:vr}, $\bm{c}_{gt}$ is the ground-truth color. 
% When ground-truth depth $z_{gt}$ is available in a training scene, we also force the mean $\mu_1$ of the first logistics distribution to be similar to the ground truth depth by a depth loss $\ell_{depth}$
% \begin{equation}
%     \ell_{depth}=\sum \|\mu_1 - z_{gt}\|^2.
% \end{equation}
% Note such a depth loss is only used in training the generalization model but not used in scene-specific training.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image_new/memory.pdf}
    \caption{Illustration for the memory interpretation. All views are input reference views. (a) During finetuning, when rendering view A using view B, C, and D, the predicted hitting probabilities and the corresponding visibility will be memorized on view A. (b) The memorized visibility on view A will be used for occlusion inference in rendering view D.}
    \label{fig:memory}
\end{figure}

\subsection{Finetune with NeuRay}
\label{sec:ft}
\textbf{Pipeline}. When finetuning NeuRay on a scene, we first use the initialization network to produce visibility features $\bm{G}'$ for all reference views. Then, the initialization network is discarded and all visibility features $\bm{G}'$ are treated as a set of trainable parameters, which are optimized along with all other networks. We randomly select an reference view in the scene as a query view and use the other reference views to render the selected pseudo query view for training. 

\textbf{Loss}. Besides the rendering loss, we use a consistency loss in the scene-specific finetuning. Since the pseudo query view is also an reference view during finetuning, every query ray has an occlusion probability $t(z)$ which can be used in computing a new hitting probability $\tilde{h}_i$ on any sample point $\bm{p}_i$ by
\begin{equation}
    \tilde{h}_i = t(z_{i+1}) - t(z_i),
\end{equation}
where $z_i$ is the depth of the point.
Thus, we can enforce the consistency between $\tilde{h}_i$ and $h_i$ in Eq.~\ref{eq:prod}, which is computed from neighboring views, to construct a consistency loss
\begin{equation}
    \ell_{consist}=\frac{1}{K_q}\sum_{i=1}^{K_q} CE(\tilde{h}_i,h_i),
\end{equation}
where $CE$ is the cross entropy loss.

\textbf{Memory interpretation}. $\ell_{consist}$ enables the network to memorize the predicted surfaces in NeuRay for occlusion inference. An example is shown in Fig.~\ref{fig:memory}.
\begin{enumerate}[leftmargin=11pt]
    \setlength{\itemsep}{1pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}
    \setlength{\itemindent}{0pt}
    \item In Fig.~\ref{fig:memory} (a), the network checks the local feature consistency of neighboring views B, C and D to predict $h_{i}$ of the query ray on the query view A.
    \item  Applying the consistency loss $\ell_{consist}$ forces the trainable visibility feature $\bm{g}$ of the query ray of A to produce $\tilde{h}_i$ consistent with $h_i$. This can be interpreted that the $h_i$ is memorized in $\bm{g}$, which also means the memorization of visibility, because both are computed from $t(z)$.
    \item  When using view A, B and C to render view D, NeuRay already knows that green point in Fig.~\ref{fig:memory} (b) is invisible to A by checking the memorized visibility on A. Thus, NeuRay overcomes the view inconsistency caused by occlusions and predicts an accurate $h$ for view D.
    \item  The predicted $h_i$ on the query ray of view D is also memorized on D and improve the $h$-prediction of other views.
\end{enumerate}

Such a memorization mechanism enables the network to refine the NeuRay representation better and better during finetuning. In contrast, existing methods~\cite{wang2021ibrnet,chibane2021stereo,Yu20arxiv_pixelNeRF} can only refine the network parameters during finetuning, which still are oblivious to occlusions.

\subsection{Speeding up rendering with NeuRay}
\label{sec:speed}
On a query ray, most sampled points $\bm{p}_i$ has zero hitting probabilities $h_i$ and thus do not affect the output color. However, most computation are wasted on these empty points. In the following, we show that a coarse hitting probability $\hat{h}_i$ can be computed from NeuRay using little computation. 
% Thus, points with small hitting probabilities will be discarded and only a small number of retained points will be fed into the subsequent networks $(M,B,P)$ to compute the output color, which speed up the rendering.
Then, to speeds up the rendering, only very few fine points are sampled around points with large $\hat{h}_i$ and are subsequently fed into the local feature matching networks $(M,B,P)$ to compute colors.

To compute the hitting probability $\hat{h}_i$, we first define the alpha value $\tilde{e}$ in depth range $(z_0,z_1)$ on a reference ray by
\begin{equation}
    \tilde{e}(z_0,z_1)=\frac{t(z_1)-t(z_0)}{1-t(z_0)}.
\end{equation}
Then, we compute the $\hat{h}_i$ on a sample point $\bm{p}_i$ by
\begin{equation}
    \hat{e}_{i}=\frac{\sum_{j}\tilde{e}_{i,j}(z_{i,j},z_{i,j}+l_i) v_{i,j}}{\sum_{j} v_{i,j}},
    \label{eq:que_exist}
\end{equation}
\begin{equation}
    \hat{h}_{i}=\prod_{k=1}^{i-1} (1-\hat{e}_k)\hat{e}_i,
\end{equation}
where $l_i=z_{i+1}-z_i$ is the distance between the point $\bm{p}_i$ and its subsequent point $\bm{p}_{i+1}$ on the query ray. Computation of $\hat{h}$ is very fast because it only involves a simple combination of $t(z)$ of reference views. We discuss the rationale behind the design of $\tilde{e}$, $\hat{e}$ and $\hat{h}$ and their connections to NeRF\cite{mildenhall2020nerf}-style density in supplementary materials.

% $\hat{h}$ is directly computed from NeuRay with a simple combination of probabilities, which is much efficient than being predicted from networks $(M,B,P)$. 

% \ly{Explanation on formulation.}

% To further speed up the computation of probability $t(z)$, we compute all distribution parameters $\mu_i$, $\sigma_i$ and $w_i$ on reference views beforehand once and directly interpolate on these distribution parameters to avoid querying network $\phi$. 

==> 02_method_bak2.tex <==
\section{Method}

Given $N$ input views of a scene with known camera poses, called \textit{reference views}, our goal is to render images from arbitrary novel views, called \textit{query views}. A camera ray is parameterized by $\bm{p}(z) =\bm{o}+z\bm{r}$, $z\in \mathbb{R}^{+}$, where $\bm{o}$ is the start point at the camera center, and $\bm{r}$ is the unit direction vector of the ray. Given a camera ray called \textit{query ray} emitting from a pixel on the query view, we sample $K_q$ points $\{\bm{p}_i \equiv \bm{p}(z_i) |i=1,...,K_q\}$ with the increasing depth $z_i$ along the ray to compute the color for the pixel. In the following, we introduce our visibility construction in NeuRay in Sec.~\ref{sec:neuray}. Then, we compute the colors and the alpha values defined on these sample points $\bm{p}_i$ by an occlusion-aware stereo matching in Sec.~\ref{sec:stereo}. 
Finally, the alpha values and colors are used in the volume rendering in Sec.~\ref{sec:vr}.

\subsection{NeuRay representation}
\label{sec:neuray}
The target of NeuRay is to encode visibility. To achieve this, we represent the scene geometry with so-called \textit{reference rays} emitting from reference views. We associate a visibility feature vector $\bm{g}\in \mathbb{R}^C$ on every reference ray to encode a visibility function $v(z)$, which means the probability that a point at depth $z$ is visible or not for this reference ray. Obviously, a valid visibility function $v(z)$ should be non-increasing on $z$ and $0\le v(z)\le 1$. 
In the following, we introduce how to compute visibility from $\bm{g}$ and then illustrate how to generate $\bm{g}$ in Sec.~\ref{sec:gen} and Sec.~\ref{sec:ft}.

The visibility is computed based on a Cumulative Density Function (CDF) $t(z)$ by $v(z)=1-t(z)$. 
As a CDF, $t(z)$ is non-decreasing from 0 to 1 so that $1-t(z)$ forms a valid visibility function. 
$t(z)$ actually corresponds to an \textit{occlusion probability} that the ray is occluded before a depth $z$ and $t(z_i)-t(z_{i-1})$ is a hitting probability that the ray hits a surface in the range $(z_{i-1},z_{i})$. 
We parameterize $t(z)$ by a mixture of logistics distributions,
\begin{equation}
    t(z;\{\mu_i,\sigma_i,w_i\})=\sum_i^{N_{l}} w_i S((z-\mu_i)/\sigma_i),
\end{equation}
where we mix $N_{l}$ logistics distributions, $\mu_i$ is the mean of $i$-th logistics distribution, $\sigma_i$ the standard deviation, $w_i$ the mixing weight with $\sum_i w_i=1$, $S(\cdot)$ a sigmoid function. All parameters $[\mu_i,\sigma_i,w_i]$ are decoded from the visibility feature $\bm{g}$ by a MLP $\phi$. In general, a ray will only hit one surface so one logistics distribution will be enough. However, using a mixture of logistics distributions improves performance when the ray hits on semi-transparent surfaces or edges of surfaces as shown in ablation studies. 

\textbf{Discussion}. An alternative way to parameterize visibility is to adapt the NeRF~\cite{mildenhall2020nerf}-like density. However, such a formulation is computationally intractable. In this density-based formulation, we directly decode a density $d(z)=\phi(z;\bm{g})$ from $\bm{g}$ using a MLP $\phi$. To compute the visibility $v(z)$, we need to first sample $K_r$ depth $\{z_k\}$ with $z_k<z$, compute their densities $d(z_k)$ and the corresponding alpha values $\alpha_{k}=1-\exp(-{\rm ReLU}(d_k))$, and finally get visibility $v(z)=\prod_{k=1}^{K_r} (1-\alpha_k)$. Though the formulation is also a valid visibility function, it is computationally infeasible because it requires $K_r$ times evaluation of $\phi$ to compute the visibility of a reference view to a point. In contrast, the visibility can be computed from a single evaluation of the network $\phi$ in our probability-based formulation. We provide more explanation in the supplementary material.

\subsection{Occlusion-aware stereo matching}
\label{sec:stereo}
We combine the visibility of NeuRay with stereo matching based methods~\cite{wang2021ibrnet,Yu20arxiv_pixelNeRF,chibane2021stereo,Trevithick20arxiv_GRF} to compute the alpha value $\alpha_i$ and the color $\bm{c}_i$ of a sample point $\bm{p}_i$. As shown in Fig.~\ref{fig:proj}, we first aggregate local features and visibilities from reference views by 
\begin{equation}
    \bm{f}_i = M (\{[\bm{f}_{i,j};v_{i,j}(z_{i,j})]|j=1,...,N\}),
    \label{eq:agg}
\end{equation}
where $\bm{f}_{i,j}$ is the local image feature of the sample point $\bm{p}_i$ projected on the $j$-th reference view, $v_{i,j}(z_{i,j})$ is the visibility from the $j$-th reference view to $\bm{p}_i$, $z_{i,j}$ is the depth of $\bm{p}_i$ on the $j$-th reference view, $M$ is a network which aggregates features and visibilities from input views to produce a feature vector $\bm{f}_i$. Then, the alpha value $\alpha_i$ and the color $\bm{c}_i$ is computed by
\begin{equation}
    \alpha_i = P (\bm{f}_i),
\end{equation}
\begin{equation}
    \bm{c}_i = B (\bm{f}_i,\{\bm{f}_{i,j};\bm{r}_{i,j} - \bm{r}_i;\bm{c}_{i,j};v_{i,j}(z_{i,j})\}),
\end{equation}
where $P$ is an alpha network which processes $\bm{f}_i$ to output the alpha value $\alpha_i$, $B$ is a color network which predicts color $\bm{c}_i$ from the feature $\bm{f}_i$, the set of features $\bm{f}_{i,j}$, view direction differences $\bm{r}_{i,j}-\bm{r}_i$ and colors $\bm{c}_{i,j}$, $\bm{r}_{i,j}$ is the view direction from $j$-th reference view to the point $\bm{p}_i$ and $\bm{c}_{i,j}$ is the color of this point projected on the reference view. The network $P$ will learn to assign a large alpha value $\alpha_i$ for $\bm{p}_i$ when local image features $\{\bm{f}_{i,j}\}$ of all visible reference views are consistent. Meanwhile, the network $B$ will learn to use the color $\bm{c}_{i,j}$ from visible reference views to produce the color $\bm{c}_i$ on $\bm{p}_i$. 
Due to the utilization of visibility, the so-called feature matching networks $(M,B,P)$ will only consider the visible views for stereo matching so that they are able to correctly compute alpha values and compute colors with the existence of occlusions. In implementation, to render a query view, we actually use $N_w$ neighboring reference views as working views in the computation.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image_new/matching_rendering.pdf}
    \caption{In occlusion-aware stereo matching, we aggregate local features, colors and visibility of reference views to compute alpha values and colors of sample points on the query ray.}
    \label{fig:proj}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{image_new/pipeline_final.pdf}
    \caption{Pipeline of rendering with NeuRay representation. Given input reference views, we compute initialized visibility features $\bm{G}'$ by a cost volume construction and an initialization network. The initialized visibility features are refined by a visibility encoder and further used in the decoder $\phi$ to compute visibility. The visibility along with local image features and colors are aggregated by the feature matching networks $M,B,P$ to compute colors and alpha values of sample points on a query ray. Finally, based on the colors and alpha values, the volume rendering is used to compute the output color of the pixel associated on the query ray.}
    \label{fig:pipeline}
\end{figure*}

\subsection{Volume rendering}
\label{sec:vr}
Given the sample points $\{\bm{p}(z_i) |i=1,...,K_q\}$ on the query ray and their alpha values $\alpha_i$, we compute the hitting probability $h_{i}$ that the ray is not occluded by any depth up to the depth $z_i$ and hits a surface in the range $(z_i,z_{i+1})$ by
\begin{equation}
    h_{i}=\prod_{k=1}^{i-1} (1-\alpha_k)\alpha_i.
    \label{eq:prod}
\end{equation}
Then, following the ray casting approach, the color for the associated pixel of the query ray is computed by
\begin{equation}
    \bm{c}_o=\sum_{i=1}^K \bm{c}_{i} h_{i},
    \label{eq:vr}
\end{equation}
where $\bm{c}_o\in \mathbb{R}^3$ is the output color for the pixel, $\bm{c}_{i}$ the color of the sample point $\bm{p}_i$. We repeat the process on every pixel on a query view to synthesize the image of the query view.

\subsection{Generalize with NeuRay}
\label{sec:gen}
To generate the visibility feature $\bm{g}$ in an unseen scene, we construct a cost volume in the view frustum of reference views, which provides a coarse estimation of surface locations for the initialization of visibility in NeuRay. As shown in Fig.~\ref{fig:pipeline}, for every reference view with its $N_s$ neighboring reference views, we compute their image feature consistency in the view frustum to construct a cost volume with size $H/4 \times W/4 \times D$~\cite{yao2018mvsnet}, where $(H,W)$ is the image size and $D$ is the number of depth planes. Then, a CNN called initialization network processes the cost volume and image features to output a visibility feature map $\bm{G}'$. Such a visibility feature map is further concatenated with image features and processed by another CNN, called visibility encoder, to produce a refined visibility feature map $\bm{G}\in \mathbb{R}^{H/4\times W/4\times C}$. Finally, the visibility feature vector $\bm{g}\in \mathbb{R}^C$ for a reference ray on this view is computed by bilinear interpolation on the feature map $\bm{G}$. Based on $\bm{g}$, visibility is decoded as in Sec.~\ref{sec:neuray}, which is subsequently used in the occlusion-aware stereo matching in Sec.~\ref{sec:stereo} and the volume rendering in Sec.~\ref{sec:vr} to synthesize images of query views. In the supplementary, we also discuss an alternative way to synthesize images without feature matching networks $(M,B,P)$.

% \textbf{Pipeline}. 
% To generate the visibility feature $\bm{g}$, we construct a cost volume in the view frustum of reference views, which provides a coarse estimation of surface locations for the initialization of visibility in NeuRay, so that NeuRay is able to generalize to unseen scenes. 
% The pipeline is shown in Fig.~\ref{fig:pipeline}. 
% For every reference view with its $N_s$ neighboring reference views, we compute their feature consistency in the view frustum to construct a cost volume with size $H\times W \times D$~\cite{yao2018mvsnet}. Then, an initialization network processes the cost volume and image features to output a visibility feature map $\bm{G}'$. Such a visibility feature map is concatenated with image features and processed by another CNN, called visibility encoder, to produce a refined visibility feature map $\bm{G}\in \mathbb{R}^{H\times W\times C}$. The initialized feature vector $\bm{g}\in \mathbb{R}^C$ for a specific reference ray is computed by bilinear interpolation on the feature map $\bm{G}$, which is subsequently utilized by the decoder MLP $\phi$ to compute the visibility (Sec.~\ref{sec:neuray}). Finally, on every sample point, visibilities, colors and local features from all reference views are aggregated by feature matching networks $(M,B,P)$ to produce a alpha value and a color (Sec.~\ref{sec:stereo}), which are finally processed by the volume rendering to compute the output color (Sec.~\ref{sec:vr}). 
% Optionally, we can replace the cost volume construction with the patch match stereo~\cite{schonberger2016pixelwise} to estimate a coarse depth map and feed the estimated depth to the initialization network to initialize NeuRay. 


\textbf{Loss}. To train the generalization model, we randomly select a query view and some reference views in a training scene to render the query view with a render loss
\begin{equation}
    \ell_{render}=\sum \|\bm{c}_{o} - \bm{c}_{gt}\|^2,
\end{equation}
where $\bm{c}_{o}$ is computed by Eq.~\ref{eq:vr}, $\bm{c}_{gt}$ is the ground-truth color. 
% When ground-truth depth $z_{gt}$ is available in a training scene, we also force the mean $\mu_1$ of the first logistics distribution to be similar to the ground truth depth by a depth loss $\ell_{depth}$
% \begin{equation}
%     \ell_{depth}=\sum \|\mu_1 - z_{gt}\|^2.
% \end{equation}
% Note such a depth loss is only used in training the generalization model but not used in scene-specific training.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image_new/memory.pdf}
    \caption{(a) During finetuning, when rendering the pseudo query view A using view B, C, and D, the predicted hitting probabilities and the corresponding visibility will be memorized on view A. (b) Afterwards, the memorized visibility on view A will be used for occlusion inference in rendering the pseudo query view D.}
    \label{fig:memory}
\end{figure}

\subsection{Finetune with NeuRay}
\label{sec:ft}
\textbf{Pipeline}. When finetuning NeuRay on a scene, we first use the initialization network to produce initial values of visibility features $\bm{G}'$ for all reference views. Then, the initialization network is discarded and visibility features $\bm{G}'$ on all reference views are treated as a set of trainable parameters, which are optimized along with all other networks. In each training step, we randomly select a reference view in the scene as a pseudo query view and use the other reference views to render the pseudo query view for training. 

\textbf{Loss}. Besides the rendering loss, we use a consistency loss in the scene-specific finetuning. Since the pseudo query view is also an reference view during finetuning, every query ray has an occlusion probability $t(z)$ which enables to compute a new hitting probability $\tilde{h}_i$ on any sample point $\bm{p}_i$ on the pseudo query ray by
\begin{equation}
    \tilde{h}_i = t(z_{i+1}) - t(z_i),
\end{equation}
where $z_i$ is the depth of the $i$-th sample point on the pseudo query view.
Thus, we can enforce the consistency between the $\tilde{h}_i$ directly decoded from NeuRay and the $h_i$ computed from neighboring reference views by occlusion-aware stereo matching in Eq.~\ref{eq:prod}, which results in a consistency loss
\begin{equation}
    \ell_{consist}=\frac{1}{K_q}\sum_{i=1}^{K_q} CE(\tilde{h}_i,h_i),
\end{equation}
where $CE$ is the cross entropy loss.

\textbf{Memorization of scene geometry}. $\ell_{consist}$ enables the network to memorize the predicted surfaces in NeuRay for occlusion inference. An example is shown in Fig.~\ref{fig:memory}.
\begin{enumerate}[leftmargin=11pt]
    \setlength{\itemsep}{1pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}
    \setlength{\itemindent}{0pt}
    \item In one training step as shown in Fig.~\ref{fig:memory} (a), NeuRay chooses A as the pseudo query view and checks the local feature consistency of neighboring views B, C and D to predict $h_{i}$ of the query ray on the query view A.
    \item  Applying the consistency loss $\ell_{consist}$ forces the trainable visibility feature $\bm{g}$ of the query ray of A to produce $\tilde{h}_i$ consistent with $h_i$. This can be interpreted that the $h_i$ is memorized in $\bm{g}$, which also means the memorization of visibility, because both are computed from $t(z)$.
    \item  In subsequent another training step which uses view A, B and C to render the pseudo query view D in Fig.~\ref{fig:memory} (b), NeuRay already knows that green point is invisible to A by checking the memorized visibility on A. Hence, NeuRay is able to predict an accurate $h_i$ for view D.
    \item  The predicted $h_i$ on the query ray of view D is also memorized on D and improve the $h$-prediction of other views in the subsequent training steps.
\end{enumerate}

By memorizing the scene geometry encoded in $h_i$, NeuRay is able to refine its representation better and better during finetuning. In contrast, existing methods~\cite{Trevithick20arxiv_GRF,wang2021ibrnet,chibane2021stereo,Yu20arxiv_pixelNeRF} can only adjust their network parameters to improve their feature matching for the scene during finetuning, which are still oblivious to occlusions in the scene.

\subsection{Speeding up rendering with NeuRay}
\label{sec:speed}
On a query ray, most sampled points $\bm{p}_i$ has zero hitting probabilities $h_i$ and thus do not affect the output color. However, most computation are wasted on these empty points. In the following, we show that a coarse hitting probability $\hat{h}_i$ can be computed from NeuRay using little computation. 
% Thus, points with small hitting probabilities will be discarded and only a small number of retained points will be fed into the subsequent networks $(M,B,P)$ to compute the output color, which speed up the rendering.
Then, to speed up the rendering, only very few fine points are sampled around points with large $\hat{h}_i$ and are subsequently fed into the feature matching networks $(M,B,P)$ to compute alpha values and colors.

To compute the hitting probability $\hat{h}_i$, we first define the alpha value $\tilde{\alpha}$ in depth range $(z_0,z_1)$ on a reference ray by
\begin{equation}
    \tilde{\alpha}(z_0,z_1)=\frac{t(z_1)-t(z_0)}{1-t(z_0)}.
\end{equation}
Then, we compute the $\hat{h}_i$ on a sample point $\bm{p}_i$ by
\begin{equation}
    \hat{\alpha}_{i}=\frac{\sum_{j}\tilde{\alpha}_{i,j}(z_{i,j},z_{i,j}+l_i) v_{i,j}(z_{i,j})}{\sum_{j} v_{i,j}(z_{i,j})},
    \label{eq:que_exist}
\end{equation}
\begin{equation}
    \hat{h}_{i}=\prod_{k=1}^{i-1} (1-\hat{\alpha}_k)\hat{\alpha}_i,
\end{equation}
where $l_i=z_{i+1}-z_i$ is the distance between the point $\bm{p}_i$ and its subsequent point $\bm{p}_{i+1}$ on the query ray. Computation of $\hat{h}$ is very fast because it only involves a simple combination of $t(z)$ of reference views. We discuss the rationale behind the design of $\tilde{\alpha}$, $\hat{\alpha}$ and $\hat{h}$ and their connections to NeRF\cite{mildenhall2020nerf}-style density in the supplementary materials.

% $\hat{h}$ is directly computed from NeuRay with a simple combination of probabilities, which is much efficient than being predicted from networks $(M,B,P)$. 

% \ly{Explanation on formulation.}

% To further speed up the computation of probability $t(z)$, we compute all distribution parameters $\mu_i$, $\sigma_i$ and $w_i$ on reference views beforehand once and directly interpolate on these distribution parameters to avoid querying network $\phi$. 

==> 02_method_bak3.tex <==

\section{Method}

Given $N$ input views of a scene with known camera poses, called \textit{reference views}, our goal is to render images from novel views, called \textit{query views}. We introduce generalization with NeuRay, finetuning with NeuRay and speeding up with NeuRay in Sec~\ref{sec:gen}, Sec~\ref{sec:ft} and Sec~\ref{sec:speed} respectively.
The whole rendering pipeline is shown in Fig.~\ref{fig:pipeline}.
First, on every reference view, we construct a cost volume to extract visibility features $\bm{G}$ on this view (Sec.~\ref{sec:vfe}). Such visibility features are used in the computation of visibility of arbitrary 3D points to this view (Sec.~\ref{sec:neuray}). Then, by considering the visibility from NeuRay, we propose an occlusion-aware radiance field construction to compute the colors and alpha values of 3D points (Sec.~\ref{sec:stereo}). The alpha values and colors are subsequently used in volume rendering for image synthesis (Sec.~\ref{sec:vr}).

\subsection{Generalize with NeuRay}
\label{sec:gen}
\subsubsection{Visibility feature extraction}
\label{sec:vfe}

For every reference view, we construct a cost volume in its view frustum to extract the visibility features $\bm{G}$. Such a cost volume encodes geometry-aware information for the visibility computation.
Specifically, we apply a CNN called image encoder to extract image features on reference views, as shown in Fig.~\ref{fig:pipeline} (a). 
Then, we sample a set of depth planes and perform the plane sweeping to warp image features from the reference view along with its $N_s$ neighboring views~\cite{yao2018mvsnet}. By computing the variance of multi-view features on each depth plane, we construct a cost volume with a size $H/4 \times W/4 \times D$, where $(H,W)$ is the image size and $D$ is the number of depth planes. 
Subsequently, a CNN called initialization network processes the cost volume to output a raw visibility feature map $\bm{G}'$. 
The raw visibility feature map is further concatenated with image features of the reference view, which are then processed by another CNN, called visibility encoder, to produce the visibility feature map $\bm{G}\in \mathbb{R}^{H/4\times W/4\times C}$. 

\vspace{-10pt}
\subsubsection{Visibility computation}
\label{sec:neuray}
To compute the visibility of a 3D point to a reference view, we consider the camera ray emitting from the reference view to the 3D point, which is called a \textit{reference ray} as shown in Fig.~\ref{fig:pipeline} (b). At the projection of the 3D point on the reference view, we bilinearly interpolate on the visibility features $\bm{G}$ to get a visibility feature vector $\bm{g}\in \mathbb{R}^C$. Then, a visibility function $v(z)$, which means the probability that a point at depth $z$ is visible or not for this reference ray, is decoded from $\bm{g}$. Obviously, a valid visibility function $v(z)$ should be non-increasing on $z$ and $v(z)\in [0,1]$. 
% The target of NeuRay is to encode visibility. To achieve this, we represent the scene geometry with so-called \textit{reference rays} emitting from reference views. 
% We associate a visibility feature vector $\bm{g}\in \mathbb{R}^C$ on every reference ray to encode a visibility function $v(z)$, which means the probability that a point at depth $z$ is visible or not for this reference ray. Obviously, a valid visibility function $v(z)$ should be non-increasing on $z$ and $0\le v(z)\le 1$. 
% In the following, we introduce how to compute visibility from $\bm{g}$ and then illustrate how to generate $\bm{g}$ in Sec.~\ref{sec:gen} and Sec.~\ref{sec:ft}.

We represent the visibility function with a Cumulative Density Function (CDF) $t(z)$ by $v(z)=1-t(z)$, which is parameterized as a mixture of logistics distributions,
\begin{equation}
    t(z;\{\mu_i,\sigma_i,w_i\})=\sum_i^{N_{l}} w_i S((z-\mu_i)/\sigma_i),
    \label{eq:occlusion}
\end{equation}
where we mix $N_{l}$ logistics distributions, $\mu_i$ is the mean of $i$-th logistics distribution, $\sigma_i$ the standard deviation, $w_i$ the mixing weight with $\sum_i w_i=1$, $S(\cdot)$ a sigmoid function. All parameters $[\mu_i,\sigma_i,w_i]=\mathcal{F}(\bm{g})$ are decoded from the feature $\bm{g}$ by an MLP $\mathcal{F}$. As a CDF, $t(z)$ is non-decreasing from 0 to 1, so that $1-t(z)$ forms a valid visibility function. 

\textbf{Physical meaning}. $t(z)$ actually corresponds to an \textit{occlusion probability} that the ray is occluded before a depth $z$ and we call the corresponding probability density function (PDF) \textit{hitting probability density}. The visibility $v(z)$ is actually the area under the PDF curve after $z$ as shown in Fig.~\ref{fig:pipeline} (b).
In general, a ray will only hit one surface so one logistics distribution will be enough. However, using a mixture of logistics distributions improves performance when the ray hits on semi-transparent surfaces or edges of surfaces as shown in ablation studies. 

\textbf{NeuRay representation}. 
Occlusion probabilities on all camera rays of all reference views together form a depiction of the scene geometry, which is exactly how a NeuRay represents the scene.
% In the generalization setting, for a particular input view, we construct its visibility feature map $\bm{G}$ as in Sec.~\ref{sec:vfe}, which is used to predict the occlusion probabilities of camera rays of this view.
The scene-specific parameters in a NeuRay representation are the raw visibility features $\bm{G}'$. In Sec.~\ref{sec:vfe}, the cost volume construction provides an initialization of $\bm{G}'$ and $\bm{G}'$ will be made trainable in the scene-specific optimization in Sec.~\ref{sec:ft}.
% The scene-specific parameters in a NeuRay representation are encoded the raw visibility features $\bm{G}'$. In the generalization setting, the cost volume construction provides an initialization of $\bm{G}'$, which is trainable in the scene-specific optimization.

\textbf{Discussion}. An alternative way to parameterize visibility $v(z)$ is to adapt the NeRF~\cite{mildenhall2020nerf}-like density. However, such a formulation is computationally impractical. In this density-based formulation, we directly decode a density $d(z)=\mathcal{F}(z;\bm{g})$ from $\bm{g}$ using an MLP $\mathcal{F}$. To compute the visibility $v(z)$, we need to first sample $K_r$ depth $\{z_k\}$ with $z_k<z$, compute their densities $d(z_k)$ and the corresponding alpha values $\alpha_{k}=1-\exp(-{\rm ReLU}(d_k))$, and finally get visibility $v(z)=\prod_{k=1}^{K_r} (1-\alpha_k)$. Though the formulation is also a valid visibility function, it is computationally infeasible because it requires $K_r$ times evaluation of $\mathcal{F}$ to compute the visibility of a reference view to a point. In contrast, the visibility can be computed from a single evaluation of the network $\mathcal{F}$ in our probability-based formulation. We provide more explanation in the supplementary material.

\vspace{-5pt}
\subsubsection{Occlusion-aware radiance field construction}
\label{sec:stereo}

We aggregate the visibility and multi-view features to construct a radiance field.
As shown in Fig.~\ref{fig:pipeline} (c), given a query view, we search for its $N_w$ neighboring reference views as working views for the feature aggregation. Specifically, for a pixel on this query view, we consider the camera ray on this pixel called \textit{query ray} parameterized by $\bm{p}(z) =\bm{o}+z\bm{r}$ where $\bm{o}$ is the camera center of the query view and $\bm{r}$ is the unit direction vector. We sample $K_q$ points $\{\bm{p}_i \equiv \bm{p}(z_i) |i=1,...,K_q\}$ with the increasing depth $z_i$ along the ray and aggregate the image features, colors and visibility from working reference views on these sample points to compute their alpha values $\alpha_i$ and colors $\bm{c}_i$.
% Given a camera ray called \textit{query ray} , $z\in \mathbb{R}^{+}$, where $\bm{o}$ is the start point at the camera center, and $\bm{r}$ is the unit direction vector of the ray, we sample $K_q$ points $\{\bm{p}_i \equiv \bm{p}(z_i) |i=1,...,K_q\}$ with the increasing depth $z_i$ along the ray to compute the color for the pixel.

On each sample point, image features from working views are first aggregated along with their visibility:
\begin{equation}
    \hat{\bm{f}}_i = \mathcal{M} (\{\bm{f}_{i,j};v_{i,j}(z_{i,j})|j=1,...,N_w\}),
    \label{eq:agg}
\end{equation}
where $\bm{f}_{i,j}$ is the image feature of the sample point $\bm{p}_i$ projected on the $j$-th reference view, $v_{i,j}(z_{i,j})$ is the visibility from the $j$-th reference view to $\bm{p}_i$, $z_{i,j}$ is the depth of $\bm{p}_i$ on the $j$-th reference view, $\mathcal{M}$ is an occlusion-aware aggregation network, $\hat{\bm{f}}_i$ is the output feature vector for $\bm{p}_i$. Then, the alpha value $\alpha_i$ is computed by
\begin{equation}
    \alpha_i = \mathcal{A} (\hat{\bm{f}}_i),
\end{equation}
where $\mathcal{A}$ is an alpha network. The color $\bm{c}_i$ is computed by
\begin{equation}
    \bm{c}_i = \mathcal{B} (\hat{\bm{f}}_i,\{\bm{f}_{i,j};\bm{r}_{i,j} - \bm{r};\bm{c}_{i,j};v_{i,j}(z_{i,j})\}),
\end{equation}
where $\mathcal{B}$ is a color blending network, $\bm{r}_{i,j}$ is the view direction from $j$-th reference view to the point $\bm{p}_i$, and $\bm{c}_{i,j}$ is the color of this point projected on the reference view. All symbols are marked in Fig.~\ref{fig:pipeline} (c) and the legend. 
The alpha network $\mathcal{A}$ will learn to assign a large alpha value $\alpha_i$ to $\bm{p}_i$ when local image features $\{\bm{f}_{i,j}\}$ of all visible reference views are consistent. 
Meanwhile, the color blending network $\mathcal{B}$ will learn to use the color $\bm{c}_{i,j}$ from visible views to produce the color $\bm{c}_i$ on $\bm{p}_i$. 
Thanks to the utilization of visibility, $(\mathcal{M},\mathcal{A},\mathcal{B})$, which we call \textit{feature aggregation networks}, will only consider the visible views for feature aggregation so that they can correctly compute alpha values and colors with the existence of occlusions.

% On each sample point, image features from working views are first aggregated along with their visibility:
% \begin{equation}
%     \bm{f}_i = M (\{[\bm{f}_{i,j};v_{i,j}(z_{i,j})]|j=1,...,N_w\}),
%     \label{eq:agg}
% \end{equation}
% where $\bm{f}_{i,j}$ is the image feature of the sample point $\bm{p}_i$ projected on the $j$-th reference view, $v_{i,j}(z_{i,j})$ is the visibility from the $j$-th reference view to $\bm{p}_i$, $z_{i,j}$ is the depth of $\bm{p}_i$ on the $j$-th reference view, $M$ is an occlusion-aware feature aggregation network, $\bm{f}_i$ is the output feature vector for $\bm{p}_i$. Then, the alpha value $\alpha_i$ and the color $\bm{c}_i$ is computed by
% \begin{equation}
%     \alpha_i = P (\bm{f}_i),
% \end{equation}
% \begin{equation}
%     \bm{c}_i = B (\bm{f}_i,\{\bm{f}_{i,j};\bm{r}_{i,j} - \bm{r};\bm{c}_{i,j};v_{i,j}(z_{i,j})\}),
% \end{equation}
% where $P$ is an alpha network which processes $\bm{f}_i$ to output the alpha value $\alpha_i$, $B$ is a color network which predicts color $\bm{c}_i$ from the feature $\bm{f}_i$, the set of features $\bm{f}_{i,j}$, view direction differences $\bm{r}_{i,j}-\bm{r}$ and colors $\bm{c}_{i,j}$, $\bm{r}_{i,j}$ is the view direction from $j$-th reference view to the point $\bm{p}_i$ and $\bm{c}_{i,j}$ is the color of this point projected on the reference view. All symbols are marked in Fig.~\ref{fig:pipeline} (c) and the legend. 
% The alpha network $P$ will learn to assign a large alpha value $\alpha_i$ to $\bm{p}_i$ when local image features $\{\bm{f}_{i,j}\}$ of all visible reference views are consistent. Meanwhile, the color network $B$ will learn to use the color $\``bm{c}_{i,j}$ from visible views to produce the color $\bm{c}_i$ on $\bm{p}_i$. 
% Due to the utilization of visibility, the feature matching networks $(M,B,P)$ will only consider the visible views for feature aggregation so that they are able to correctly compute alpha values and colors with the existence of occlusions. 

\vspace{-5pt}
\subsubsection{Volume rendering}
\label{sec:vr}
The alpha values $\alpha_i$ and colors $\bm{c}_i$ on sample points will be used in volume rendering to compute the color of the pixel on the query view. We first compute the hitting probability $h_{i}$ that the query ray is not occluded by any depth up to the depth $z_i$ and hits a surface in the range $(z_i,z_{i+1})$ by
\begin{equation}
    h_{i}=\prod_{k=1}^{i-1} (1-\alpha_k)\alpha_i.
    \label{eq:prod}
\end{equation}
Then, following \cite{mildenhall2020nerf}, the color for the associated pixel of the query ray is computed by
\begin{equation}
    \bm{c}_o=\sum_{i=1}^K \bm{c}_{i} h_{i},
    \label{eq:vr}
\end{equation}
where $\bm{c}_o\in \mathbb{R}^3$ is the output color for the pixel.
We use the volume rendering on every pixel of the query view to synthesize the image for the view.
% We apply the ray casting scheme on every pixel of the query view to synthesize the image for the view.

\textbf{Loss}. To train our model, we randomly select a training scene and choose a query view and some reference views in the scene to render the query view with a render loss
\begin{equation}
    \ell_{render}=\sum \|\bm{c}_{o} - \bm{c}_{gt}\|^2,
\end{equation}
where $\bm{c}_{gt}$ is the ground-truth color. 
% When ground-truth depth $z_{gt}$ is available in a training scene, we also force the mean $\mu_1$ of the first logistics distribution to be similar to the ground truth depth by a depth loss $\ell_{depth}$
% \begin{equation}
%     \ell_{depth}=\sum \|\mu_1 - z_{gt}\|^2.
% \end{equation}
% Note such a depth loss is only used in training the generalization model but not used in scene-specific training.


\subsection{Finetune with NeuRay}
\label{sec:ft}
% The estimated visibility of NeuRay can be further refined by scene-specific finetuning. 
The cost volume construction in Sec~\ref{sec:vfe} provides an initialization of NeuRay, which can be further refined by finetuning on a specific scene.
Specifically, in the finetuning, we first construct the cost volumes and use the initialization network to produce initial values of raw visibility features $\bm{G}'$ for all reference views. Then, the initialization network is discarded and the raw visibility features $\bm{G}'$ on all reference views are treated as a set of trainable parameters, which are optimized along with all other networks. In each training step, we randomly select a reference view in the scene as a pseudo query view and use the other reference views to render the pseudo query view for training. 

\textbf{Consistency loss}. Besides the rendering loss, we use a consistency loss in the scene-specific finetuning. Since a query ray of the pseudo query view is also a reference ray, there are two ways to compute the hitting probability of a sample point $\bm{p}_i$ on this ray. One is from the constructed radiance field, which aggregates features from neighboring workings views to compute alpha values and use Eq.~\eqref{eq:prod} to compute $h_i$. The other way is to use the occlusion probability $t(z)$ from the NeuRay representation. Specifically, on this pseudo query ray, we first predict its occlusion probability $t(z)$ using Eq.~\eqref{eq:occlusion} and then compute the hitting probability $\tilde{h}_i$ on the sampled point $\bm{p}_i$ by
\begin{equation}
    \tilde{h}_i = t(z_{i+1}) - t(z_i),
\end{equation}
where $z_i$ is the depth of the sample point $\bm{p}_i$. Thus, we can enforce the consistency between $\tilde{h}_i$ decoded from NeuRay and $h_i$ computed from the constructed radiance field, which results in a consistency loss
\begin{equation}
    \ell_{consist}=\frac{1}{K_q}\sum_{i=1}^{K_q} CE(\tilde{h}_i,h_i),
\end{equation}
where $CE$ is the cross entropy loss.

% \textbf{Loss}. Besides the rendering loss, we use a consistency loss in the scene-specific finetuning. Since the pseudo query view is also a reference view during finetuning, every query ray has an occlusion probability $t(z)$ which enables to directly compute a hitting probability $\tilde{h}_i$ on the sample point $\bm{p}_i$ on the pseudo query ray by
% \begin{equation}
%     \tilde{h}_i = t(z_{i+1}) - t(z_i),
% \end{equation}
% where $z_i$ is the depth of the $i$-th sample point on the pseudo query view.
% Thus, we can enforce the consistency between the $\tilde{h}_i$ directly decoded from NeuRay and the $h_i$ computed from neighboring reference views by occlusion-aware aggregation, which results in a consistency loss
% \begin{equation}
%     \ell_{consist}=\frac{1}{K_q}\sum_{i=1}^{K_q} CE(\tilde{h}_i,h_i),
% \end{equation}
% where $CE$ is the cross entropy loss.

\textbf{Memorization of scene geometry}. $\ell_{consist}$ enables the NeuRay representation to memorize the predicted surfaces from the constructed radiance field in finetuning. An example is shown in Fig.~\ref{fig:memory}.
\vspace{-5pt}
\begin{enumerate}[leftmargin=11pt]
    \setlength{\itemsep}{1pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}
    \setlength{\itemindent}{0pt}
    \item In one training step as shown in Fig.~\ref{fig:memory} (a), NeuRay chooses view A as the pseudo query view and aggregates features from neighboring views B, C and D to predict $h_{i}$ of the query ray on the query view A.
    \item  Applying the consistency loss $\ell_{consist}$ forces the visibility feature $\bm{g}$ of the query ray of A to produce $\tilde{h}_i$ consistent with $h_i$. This can be interpreted that the $h_i$ is memorized in $\bm{g}$, which also means the memorization of visibility, because both are computed from $t(z)$.
    \item  In subsequent another training step which uses view A, B and C to render the pseudo query view D in Fig.~\ref{fig:memory} (b), NeuRay already knows that the green point is invisible to A by checking the memorized visibility on A. Hence, NeuRay is able to predict an accurate $h_i$ for view D.
    \item  The predicted $h_i$ on the query ray of view D is also memorized on D and facilitates the prediction of hitting probabilities of other views in the subsequent training steps.
\end{enumerate}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image_new/memory.pdf}
    \caption{(a) During finetuning, when rendering the pseudo query view A using view B, C, and D, the predicted hitting probabilities and the corresponding visibility will be memorized on view A. (b) Afterwards, the memorized visibility on view A will be used for occlusion inference in rendering the pseudo query view D.}
    \vspace{-10pt}
    \label{fig:memory}
\end{figure}

By memorizing the scene geometry in $h_i$, NeuRay is able to refine its scene representation to provide better occlusion inference during finetuning. In contrast, existing methods~\cite{Trevithick20arxiv_GRF,wang2021ibrnet,chibane2021stereo,Yu20arxiv_pixelNeRF} can only adjust their network parameters to improve their feature matching during finetuning, which are still oblivious to occlusions in the scene.


\subsection{Speeding up rendering with NeuRay}

\label{sec:speed}
On a query ray, most sampled points $\bm{p}_i$ have zero hitting probabilities $h_i$ and thus do not affect the output color. 
We show that a coarse hitting probability $\hat{h}_i$ can be computed from NeuRay to filter out these empty points. 
Then, to speed up the rendering, only very few fine points are sampled around points with large $\hat{h}_i$ and are further considered in volume rendering to compute the color.

% To speed up the rendering, we show that NeuRay is able to efficiently predict a coarse hitting probabilities $\hat{h}$ of sample points on query rays of novel views. 


% In the following, we show that a coarse hitting probability $\hat{h}_i$ can be computed from NeuRay using little computation. 
% Thus, points with small hitting probabilities will be discarded and only a small number of retained points will be fed into the subsequent networks $(M,B,P)$ to compute the output color, which speed up the rendering.
% Then, to speed up the rendering, only very few points are sampled around points with large $\hat{h}_i$ and are subsequently fed into the feature matching networks $(M,B,P)$ to compute alpha values and colors.

Specifically, we first define the alpha value $\tilde{\alpha}$ in depth range $(z_0,z_1)$ on a reference ray by
% To compute the hitting probability $\hat{h}_i$, we first define the alpha value $\tilde{\alpha}$ in depth range $(z_0,z_1)$ on a reference ray by
\begin{equation}
    \tilde{\alpha}(z_0,z_1)=\frac{t(z_1)-t(z_0)}{1-t(z_0)}.
\end{equation}
Then, we compute the $\hat{h}_i$ on a sample point $\bm{p}_i$ by
\begin{equation}
    \hat{\alpha}_{i}=\frac{\sum_{j}\tilde{\alpha}_{i,j}(z_{i,j},z_{i,j}+l_i) v_{i,j}(z_{i,j})}{\sum_{j} v_{i,j}(z_{i,j})},
    \label{eq:que_exist}
\end{equation}
\begin{equation}
    \hat{h}_{i}=\prod_{k=1}^{i-1} (1-\hat{\alpha}_k)\hat{\alpha}_i,
\end{equation}
where $l_i=z_{i+1}-z_i$ is the distance between the point $\bm{p}_i$ and its subsequent point $\bm{p}_{i+1}$ on the query ray. Computation of $\hat{h}$ is very fast because it only involves a simple combination of $t(z)$ of reference views. We discuss the rationale behind the design of $\tilde{\alpha}$, $\hat{\alpha}$ and $\hat{h}$ and their connections to NeRF\cite{mildenhall2020nerf}-style density in the supplementary materials.

% $\hat{h}$ is directly computed from NeuRay with a simple combination of probabilities, which is much efficient than being predicted from networks $(M,B,P)$. 

% \ly{Explanation on formulation.}

% To further speed up the computation of probability $t(z)$, we compute all distribution parameters $\mu_i$, $\sigma_i$ and $w_i$ on reference views beforehand once and directly interpolate on these distribution parameters to avoid querying network $\phi$. 


==> image/depth_fusion.tex <==
\begin{figure}
    \centering
    \begin{tabular}{ccc}
         Image & Input depth & Optimized depth \\
         \includegraphics[width=0.3\linewidth]{image/lego_90.png} &
         \includegraphics[width=0.3\linewidth]{image/neuray_nr_ft_lego_v4-90-in.jpg} & 
         \includegraphics[width=0.3\linewidth]{image/neuray_nr_ft_lego_v4-90.jpg} \\
         \includegraphics[width=0.3\linewidth]{image/hotdog_31.png} &
         \includegraphics[width=0.3\linewidth]{image/neuray_nr_ft_hotdog_v2-13-in.jpg} & 
         \includegraphics[width=0.3\linewidth]{image/neuray_nr_ft_hotdog_v2-13.jpg} \\
         \includegraphics[width=0.3\linewidth]{image/drums_63.png} &
         \includegraphics[width=0.3\linewidth]{image/neuray_nr_ft_drums_v2-63-in.jpg} & 
         \includegraphics[width=0.3\linewidth]{image/neuray_nr_ft_drums_v2-63.jpg} 
    \end{tabular}
    \caption{Input depth maps estimated by Colmap~\cite{schoenberger2016mvs} and optimized depth maps by NeuRay on the same reference views. The optimized depth values are the means $\mu$ of all reference rays. In the input depth map, there are white regions which are the failed regions for the external MVS algorithm. Optimizing NeuRay representation can find correct depth values for these failed regions. Note backgrounds are masked out for clear visualization.}
    \label{fig:depth_fusion}
\end{figure}

==> image/finetune.tex <==
\begin{figure*}
    \centering
    \begin{tabular}{ccccc}
    Ground-truth & NeuRay-DR & NeuRay-NR & IBRNet & NeRF \\
    \includegraphics[width=\imgsize\linewidth]{image/finetune/ft-gt-hotdog-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/finetune/ft-dr-hotdog-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/finetune/ft-nr-hotdog-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/finetune/ft-ibrnet-hotdog-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/finetune/ft-nerf-hotdog-0.png} \\
    \includegraphics[width=\imgsize\linewidth]{image/finetune/ft-gt-mic-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/finetune/ft-dr-mic-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/finetune/ft-nr-mic-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/finetune/ft-ibrnet-mic-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/finetune/ft-nerf-mic-0.png} \\
    \includegraphics[width=\imgsize\linewidth]{image/finetune/ft-gt-ship-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/finetune/ft-dr-ship-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/finetune/ft-nr-ship-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/finetune/ft-ibrnet-ship-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/finetune/ft-nerf-ship-0.png} \\
    \end{tabular}
    \caption{Results in the finetuning setting. All models are trained on the scene for 10k steps. NeRF is trained from scratch while NeuRay and IBRNet are first initialized by their generalization models.}
    \label{fig:finetune}
\end{figure*}

==> image/generalization.tex <==

\begin{figure*}
    \centering
    \begin{tabular}{ccccc}
    Ground-truth & NeuRay-DR & NeuRay-NR & IBRNet & PixelNeRF \\
    \includegraphics[width=\imgsize\linewidth]{image/generalization/gen-gt-lego-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/generalization/gen-dr-lego-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/generalization/gen-nr-lego-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/generalization/gen-ibrnet-lego-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/generalization/gen-pixel_nerf-lego-0.png} \\
    \includegraphics[width=\imgsize\linewidth]{image/generalization/gen-gt-chair-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/generalization/gen-dr-chair-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/generalization/gen-nr-chair-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/generalization/gen-ibrnet-chair-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/generalization/gen-pixel_nerf-chair-0.png} \\
    \includegraphics[width=\imgsize\linewidth]{image/generalization/gen-gt-drums-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/generalization/gen-dr-drums-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/generalization/gen-nr-drums-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/generalization/gen-ibrnet-drums-0.png} &
    \includegraphics[width=\imgsize\linewidth]{image/generalization/gen-pixel_nerf-drums-0.png} \\
    \end{tabular}
    \caption{Qualitative results in the generalization setting. NeuRay performs better in regions with severe self-occlusion, e.g. the plane occluded by arms of Lego model, the chair plane occluded by the arm of the chair and the center region of drums.}
    \label{fig:gen}
\end{figure*}

==> image/in_view_num.tex <==
\begin{figure*}
    \centering
    \begin{tabular}{ccccc}
         \#Input view=25 & \#Input view=50 & \#Input view=75 & \#Input view=100 & Ground Truth \\
         \includegraphics[width=\imgsize\textwidth]{image/in_num/25-lego.png} &
         \includegraphics[width=\imgsize\textwidth]{image/in_num/50-lego.png}&
         \includegraphics[width=\imgsize\textwidth]{image/in_num/75-lego.png}&
         \includegraphics[width=\imgsize\textwidth]{image/in_num/100-lego.png}&
         \includegraphics[width=\imgsize\textwidth]{image/in_num/gt-lego.png}
    \end{tabular}
    \caption{Qualitative results of NeuRay-NR in the generalization setting using different input view numbers. With only 25 input views around the scene, obvious artifacts appear since the supporting neighboring view is too far from the query view. When there are 50 input views, NeuRay is already able to produce rendering images of satisfactory quality.}
    \label{fig:in_view_num}
\end{figure*}

==> image/progress.tex <==

\begin{figure*}
    \centering
    \begin{tabular}{ccccc}
    PSNR Curves & Ground-Truth & IBRNet-Ft & NeuRay-DR-Ft & NeuRay-NR-Ft  \\
    \includegraphics[width=0.22\textwidth]{image/progress.pdf} & 
    \includegraphics[width=0.17\textwidth]{image/progress/gt-lego-step-10k.png}& 
    \includegraphics[width=0.17\textwidth]{image/progress/ibrnet-lego-step-10k.png}& 
    \includegraphics[width=0.17\textwidth]{image/progress/dr-lego-step-10k.png}& 
    \includegraphics[width=0.17\textwidth]{image/progress/nr-lego-step-10k.png} 
    \end{tabular}
    \caption{Curves of PSNR on different steps and qualitative results on the 100k steps. Note the PSNR is computed on a validation set with 6 images.}
    \label{fig:progress}
\end{figure*}

==> image/specifc.tex <==
\newcommand\imgsize{0.18}
\begin{figure*}
    \centering
    \begin{tabular}{ccccc}
    % whole, GT, | DR, NR, NeRF, | DR-Init, NR-Init, IBRNet, PixelNeRF | NeRF, DR-ft, NR-ft, IBRNet-ft
    & Ground-truth & NeuRay-DR & NeuRay-NR & NeRF \\
    \includegraphics[width=\imgsize\textwidth]{image/specific/gt-lego-0.png} &
    \includegraphics[width=\imgsize\textwidth]{image/specific/gt-lego-0-part.png} &
    \includegraphics[width=\imgsize\textwidth]{image/specific/dr-lego-0-part.png} &
    \includegraphics[width=\imgsize\textwidth]{image/specific/nr-lego-0-part.png} &
    \includegraphics[width=\imgsize\textwidth]{image/specific/nerf-lego-0-part.png} \\
    \includegraphics[width=\imgsize\textwidth]{image/specific/gt-drums-0.png} &
    \includegraphics[width=\imgsize\textwidth]{image/specific/gt-drums-0-part.png} &
    \includegraphics[width=\imgsize\textwidth]{image/specific/dr-drums-0-part.png} &
    \includegraphics[width=\imgsize\textwidth]{image/specific/nr-drums-0-part.png} &
    \includegraphics[width=\imgsize\textwidth]{image/specific/nerf-drums-0-part.png} \\
    \includegraphics[width=\imgsize\textwidth]{image/specific/gt-materials-0.png} &
    \includegraphics[width=\imgsize\textwidth]{image/specific/gt-materials-0-part.png} &
    \includegraphics[width=\imgsize\textwidth]{image/specific/dr-materials-0-part.png} &
    \includegraphics[width=\imgsize\textwidth]{image/specific/nr-materials-0-part.png} &
    \includegraphics[width=\imgsize\textwidth]{image/specific/nerf-materials-0-part.png} \\
    \end{tabular}
    \caption{Qualitative results in the scene-specific training with 200k training steps. NeuRay can recover the subtle regions, like the texture on the Lego, the transparent drum surface or the reflective materials, more clearly than NeRF with the same training steps.}
    \label{fig:scene}
\end{figure*}

==> image/work_view_num.tex <==

\begin{figure}
    \centering
    \begin{tabular}{cc}
         \includegraphics[width=0.45\linewidth]{image/in_vn.pdf} &
         \includegraphics[width=0.45\linewidth]{image/work_num.pdf} \\
         (a) & (b)
    \end{tabular}
    \caption{PSNR of NeuRay on the Lego using different numbers of input view (a) or different numbers of working view (b). "Gen" means the generalization setting while "Ft" means the finetuning setting with 100k steps.}
    \label{fig:view_num}
\end{figure}

==> table/high_res.tex <==
\begin{table}
    \centering
    \caption{PSNRs on the NeRF-synthetic dataset with resolution of 800$\times$800 and the forward-facing LLFF dataset with resolution of 1008$\times$756.}
    
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccc}
    \toprule
    
     \multirow{2}{*}{Setting} & \multirow{2}{*}{Method}   & \multicolumn{2}{c}{Dataset}  \\
     & & NeRF-Synthetic & Forward-Facing \\
     \midrule
     \multirow{4}{*}{Generalization} 
     &MVSNeRF   &  22.67   & 17.56\\
     &LLFF      &  24.88   & 24.13\\
     &IBRNet    &  25.49   &  25.13\\
     &NeuRay    &  \textbf{27.24}   & \textbf{25.15}\\
     \midrule
     \multirow{4}{*}{Finetune} 
     &MVSNeRF   & 27.21  & 26.25\\
     &IBRNet    & 28.14  & 26.73\\
     &NeRF      & 31.01  & 26.50\\
     &NeuRay    & \textbf{32.42}  &  \textbf{26.78} \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:high_res}
\end{table}

==> table/low_res.tex <==
\begin{table*}
    \centering
    \caption{PSNRs on the NeRF-synthetic dataset with resolution of 800$\times$800 and the forward-facing LLFF dataset with resolution of 1008$\times$756.}
    
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccc}
    \toprule
    
     \multirow{2}{*}{Setting} & \multirow{2}{*}{Method}   & \multicolumn{2}{c}{Dataset}  \\
     & & NeRF-Synthetic & Forward-Facing \\
     \midrule
     \multirow{4}{*}{Generalization} 
     &MVSNeRF   &  22.67   & 17.56\\
     &LLFF      &  24.88   & 24.13\\
     &IBRNet    &  25.49   &  25.13\\
     &NeuRay    &  \textbf{27.24}   & \textbf{25.15}\\
     \midrule
     \multirow{4}{*}{Finetune} 
     &MVSNeRF   & 27.21  & 26.25\\
     &IBRNet    & 28.14  & 26.73\\
     &NeRF      & 31.01  & 26.50\\
     &NeuRay    & \textbf{32.42}  &  \textbf{26.78} \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:high_res}
\end{table*}
